The Study of a Fibre Z-Pinch

This thesis presents the results of fibre Z-pinch experiments carried out on the Z-150 device at the CTU in Prague. The generator that was used to drive the experiments consisted of one capacitor of 3e-6 F capacitance. In the case of 20 kV charging voltage, the current was peaking at 80 kA with a 850 ns quarter period. The Z-pinch was formed from carbon fibres of 15 micrometer diameter and 1 cm length. The discharge was observed by a large number of diagnostic tools. This comprehensive set of diagnostics enabled us to describe the gross dynamics of the Z-pinch. It was found out that after the breakdown a low density coronal plasma was formed while the fibre diameter remained almost unchanged. This low density corona was carrying almost all the current of the order of 10 kA. When the current had built up, the implosion of the corona onto the central fibre occurred. The implosion velocity approached the value of 2e5 m/s. When the imploded corona had reached the fibre, the dip in dI/dt, voltage peak up to 10 kV, and XUV pulse of a 10-30 ns width were observed. XUV radiation was emitted from several bright spots which corresponded to the interaction of m=0 instability necks with the dense core. The electron temperature and density were approximately 80 eV and 10e25 per cubic meter, respectively. Although the presence of a fibre did not significantly suppress MHD instabilities, they were not disruptive. After the fibre ablation, i.e. after 500 ns, material evaporated from electrodes started to play a dominant role. The observed plasma column seemed to be MHD unstable and when m=0 instabilities had developed, X-ray pulses were emitted from several hot spots, particularly near the anode. At that time the voltage peak of up to 30 kV was detected.

==> spectroscopy.tex <==
\section{Applied spectroscopic methods}
The basic theory of emission spectroscopy will be introduced in
this section so as we could describe the spectroscopic methods. As
there are numerous spectroscopic methods \citep{Griem64, Griem74,
Hauer91, Griem97, Thorne99} we will deal only with those that were
used in our experiment.

\subsection{Introduction}
The characteristic property of plasma is its radiating in a
broadband spectral region. Therefore emission spectroscopy is a
diagnostic technique that has been applied to an evaluation of
appropriate plasma parameters since the very beginning of plasma
physics \citep{Griem64,deMichelis81}. By emission spectroscopy it
is possible to measure
 plasma composition,  electron temperature and density,
 ion temperature and density, electric and magnetic
field, plasma motion or turbulence, plasma dynamics, ionization
dynamics, etc~\citep{Kunze89}. The measurement of these quantities
is possible provided that transition probabilities (i.e.
oscillator strengths), and collision cross--sections are
known\footnote{On the contrary to that if we determine plasma
parameters by other non--spectroscopic methods, e.g. by laser
interferometry and laser scattering, we can experimentally measure
or verify transition probabilities or collision cross--sections.
This experimental measurement is still needed~\citep{Kunze02}.}.

As the temperature of $Z$--pinches varies from several eVs up to
tens of keV, a predominant fraction of the electromagnetic
radiation is emitted in XUV and X--ray spectral region. The
boundaries of XUV and X--ray ranges are not all rigid, but are
those traditionally accepted in the fields of X--ray spectroscopy,
plasma physics, astrophysics, X--ray laser etc. For the purpose of
this paper, we used the following wavelength
ranges~\citep{Pikuz01}

\begin{figure}
\center{
\begin{tabular}{|l|l|}
\hline \hline Spectral region& Wavelength  \\
\hline
X--ray & 0.01~nm $\div$ 2.5 nm \\
\hline
hard X--ray & 0.01~nm $\div$ 0.2 nm \\
\hline
soft X--ray & 0.2~nm $\div$ 2.5 nm \\
\hline
XUV & 2.5~nm $\div$ 40 nm \\
\hline
VUV & 40~nm $\div$ 200 nm \\
\hline\hline
\end{tabular}
\caption{Definition of wavelength ranges used in our work.}}
\end{figure}

\subsection{Radiative processes}
Radiative processes in a plasma can be divided into three main
groups according to the type of transition. We can distinguish
transitions between two states of electrons -- free and bound.
\begin{itemize}
\item \emph{Free--free transitions} are associated with a gain or
loss of an electron energy in the field of an
ion\footnote{Collision between two electrons cannot produce
radiation by electric or magnetic dipole processes.}.  As free
states are not quantized therefore a broad continuum radiation is
created. At long wavelengths, the free--free emission approaches
the blackbody function. The loss of the electron energy into the
radiation is connected with the deceleration of electrons and
therefore we speak about Bremsstrahlung radiation. The absorption
of a photon by an electron is called as the inverse
Bremsstrahlung.

\item \emph{Free--bound transitions} correspond to the
recombination and photoionization processes. Recombination
continuum extends from each bound state of an electron and is
characterised by edges. Similarly, the absorption edges occur in
the spectral dependence of the photoionization cross--section.

\item \emph{Bound--bound transitions} occur when an electron
bounded by an ion makes a transition to another bound state. When
the final state has lower energy than the initial one, the photon
of well--defined energy is emitted. The inverse mechanism is the
photoexcitation. The radiation is characterised by emission or
absorption spectral lines.

The rate of spontaneous emission from the upper energy level ``u''
to lower level ``l'' is defined by means of Einstein probability
coefficient $A_\mathrm{ul}$ as follows
\begin{equation}
\frac{\diff n_\mathrm{u}}{\diff t}\Bigg|_{\mathrm{u}\rightarrow
\mathrm{l}}=-A_\mathrm{{ul}} n_\mathrm{u}
\end{equation}

where $n_\mathrm{u}$ is the number density of electrons in the
upper level. The overall rate of spontaneous radiative transition
from the upper level ``u'' is given by the sum of the rates from
the upper level ``u'' to all lower levels
\begin{equation}
\frac{\diff n_\mathrm{u}}{\diff
t}=-\sum_{\mathrm{l}<\mathrm{u}}A_\mathrm{{ul}}
n_\mathrm{u}=-A_\mathrm{u\rightarrow} n_\mathrm{u}
\end{equation}

The probability of spontaneous emission $A_\mathrm{ul}$ is treated in quantum electrodynamics and is given by a
selection rules. As far as our experiments with carbon fibres are concerned, we observed only allowed
transitions with $\langle l|e\vec{r}|u\rangle\neq 0$. The transitions that can occur by magnetic dipole and
electric quadrupole were very weak since the plasma density was not sufficiently low. The intercombination lines
with $\triangle \mathbb{S}\neq 0$ are not usually observed for low--$Z$ elements, such as carbon, where the
spin--orbit interaction is small.
\end{itemize}

\subsection{Collisional processes in plasma}

\begin{figure}[!h]
\centerline{\includegraphics{./eps/procesy.png}} \captionstyle{hang} \setlength{\captionmargin}{2cm}
\caption{Several possible radiative and collisional processes. \small{(\mbox{Radiative processes are labeled by
wavy line.})}} \label{procesy}
\end{figure}

Similarly to radiative processes, we can distinguish between
collisional excitation -- de-excitation, ionization --
recombination, etc. But on the contrary to radiative processes,
collisional transitions between two states do not follow any
selection rules. The crucial collisional process in a plasma is an
\emph{interaction of a bound electron with free electrons}. The
collision of a bound electron with ions is much more less
significant due to substantial diference in mass. When a free
electron collides with an electron bounded in an ion A, excitation
or ionization of a bound electron can occur \vspace{0.2cm}

\vspace{0.2cm}
\begin{tabular}{l l l l}
 \hspace{1.5cm} A$^z+e^-$ & $\leftrightarrow$ & A$^{z*}+e^-$ &(excitation,
 de-excitation)\\[0.2cm]
 \hspace{1.5cm}  A$^z+e^-$ & $\leftrightarrow$ & A$^{z+1}+e^-+e^-$ &(ionization, three-body
 recombination) \\
\end{tabular}

\vspace{0.3cm} In three-body recombination, the inverse of
collisional ionization, an excited bound state of the ion A$^{z}$
is formed and the excess energy is given to an electron. The
cross--section of this reaction is increasing with the square of
the electron density $n_\mathrm{e}$ and is larger for transitions
into highly excited levels. On the contrary to that, the radiative
capture of an electron occurs mainly into the ground state

\vspace{0.2cm}
\begin{tabular}{l l l p{5cm}}
 \hspace{1.52cm} A$^{z+1}+e^-$ & $\rightarrow$ & A$^{z}+h\nu$ &\hspace{0.77cm} (radiative~capture) \\
\end{tabular}

\vspace{0.3cm} In the case of high--temperature and low density
plasma ($n_\mathrm{e}<10^{16}\,\mathrm{cm}^{-3}$), the dominant
recombination process is dielectronic recombination: a free
electron is resonantly captured in a high level, with simultaneous
excitation of one of the electrons of the recombining ion
A$^{z+1}$. A doubly--excited ion A$^{z**}$ is formed

\vspace{0.2cm}
\begin{tabular}{l l l l}
\hspace{1.5cm} A$^{z+1}+e^-$ & $\leftrightarrow$ & A$^{z**}$
&\hspace{1.3cm} (dielectronic recombination, autoionization)
\end{tabular}

\vspace{0.3cm} As the doubly--excited state is above the
ionization limit of the recombined ion it is unstable. The two
electron excited state can either undergo the inversion process
--- autoionization or radiatively decay by the emission of photons.

Finally we mention the charge--exchange recombination that happens
during collision between two ions or between ion and atom. When
the charge of ion A is greater than that of ion B, the electron
bounded in ion A could be captured by the other ion B into a
highly excited level

\vspace{0.2cm}
\begin{tabular}{l l l l}
\hspace{1.5cm} A$^{z_\mathrm{A}}+B^{z_\mathrm{B}}$ & $\rightarrow$
& A$^{z_\mathrm{A}-1}+B^{z_\mathrm{B}+1}$ &(charge--exchange
recombination)
\end{tabular}

\vspace{0.3cm} The quantitative description of collisional
processes begins with the cross--section $\sigma (v)$. The number
of transitions ``a'' (of an ion A induced by electrons) per unit
time and per unit volume is given by equation
\begin{equation}
R_\mathrm{a}=-\frac{\diff n_\mathrm{A}}{\diff t}=\langle\sigma
(v)\cdot v\rangle
n_\mathrm{e}n_\mathrm{A}=C_\mathrm{a}n_\mathrm{A}
\end{equation}

where $\langle\sigma (v)\cdot v\rangle=\int\sigma
(v)f_\mathrm{e}(v)v\diff v$ represent so-called rate coefficient.
The rate coefficient is calculated by averaging of $\sigma
(v)\cdot v$ over the electron velocity distribution
$f_\mathrm{e}(v)$. The excitation/deexcitation rate coefficient is
usually labeled as $X$, ionization rate coefficient as $S$, and
recombination coefficient as $\alpha$. The quantity $C_\mathrm{a}$
is called as the probability of collision of one ion A with
electrons.


\subsection{Population of energy levels}

The rate of radiative and collisional processes in plasma
determine the population of each energy level. In order to
simplify notation, the rate of all collisions filling the upper
level ``u'' will be marked as $R^\mathrm{c}_{\rightarrow
\mathrm{u}}$, similarly the rate of radiative processes will be
marked as $R^\mathrm{r}_{\rightarrow \mathrm{u}}$ and the rate of
collisions depopulating the level ``u'' as
$R^\mathrm{c}_{\mathrm{u}\rightarrow}=C_{\mathrm{u}\rightarrow}n_\mathrm{u}=X_{\mathrm{u}\rightarrow}n_\mathrm{e}n_\mathrm{u}$.
The symbol $A_{\mathrm{u}\rightarrow}$ stands for the total
transition probability for emission from the level ``u''. By using
these quantities we can write the following rate equation
\begin{equation}
\label{rychlostnirovnice} \frac{\diff n_\mathrm{u}}{\diff
t}=R^\mathrm{c}_{\rightarrow \mathrm{u}}+R^\mathrm{r}_{\rightarrow
\mathrm{u}}-R^\mathrm{c}_{\mathrm{u}\rightarrow}-A_{\mathrm{u}\rightarrow}n_\mathrm{u}
\end{equation}

Usually $n_\mathrm{e}$ and $T_\mathrm{e}$ change slowly compared
to atomic time constants
$\tau_\mathrm{u}=1/(A_{\mathrm{u}\rightarrow}+C_{\mathrm{u}\rightarrow})$.
It means that the the population density $n_\mathrm{u}$ could be
assumed to be in quasi--equilibrium where $\diff n_u/\diff t$.
Simplifying the rate equation~\ref{rychlostnirovnice} we obtain
the population of upper level in collisional--radiative
equilibrium
\begin{equation}
\label{quasiequilibrium}
 n_\mathrm{u}=\frac{R^\mathrm{c}_{\rightarrow
\mathrm{u}}+R^\mathrm{r}_{\rightarrow
\mathrm{u}}}{A_{\mathrm{u}\rightarrow}+C_{\mathrm{u}\rightarrow}}
\end{equation}

The analytic solution of any model taking into account all
processes is still too complicated and it is necessary to use
numerical simulation (For our purposes we used time--dependent
atomic physics code FLY described in appendix~\ref{appendixA}).
However, simplifications of equation~\ref{quasiequilibrium} are
still possible in two limiting cases. In the case of low density
plasma with $n_\mathrm{e}<10^{14}$~cm$^{-3}$ the population
follows the corona model. In the following we will restrict to the
other limiting case, to high density plasma in LTE (Local
Thermodynamic Equilibrium).

\subsubsection{Local thermodynamic equilibrium}

The criterion for LTE is that the collisional rates must be much
larger that radiative rates. Then the radiative terms in equation
\ref{quasiequilibrium} can be neglected and we get
\begin{equation}
\label{LTE1}
 n_\mathrm{u}=\frac{R^\mathrm{c}_{\rightarrow
\mathrm{u}}}{C_{\mathrm{u}\rightarrow}}=\frac{n_\mathrm{e}X_{\rightarrow
\mathrm{u}}}{X_{\mathrm{u}\rightarrow}}
\end{equation}

From the principle of the detailed balance\footnote{Every process
must be balanced by its exact inverse.} follows that
\begin{equation}
\label{LTE2} \frac{X_{\mathrm{l}\rightarrow
\mathrm{u}}}{X_{\mathrm{u}\rightarrow\mathrm{l}}}=\frac{g_\mathrm{u}}{g_\mathrm{l}}\mathrm{e}^{-\frac{E_\mathrm{u}-E_\mathrm{l}}{kT_\mathrm{e}}}
\end{equation}

where $g_\mathrm{u}$, $g_\mathrm{l}$ are the statistical weights
for levels with energies $E_\mathrm{u}$ and $E_\mathrm{l}$,
respectively. Applying equation \ref{LTE2} to any two levels in
atomic species and combining it with equation~\ref{LTE1} it is
possible to derive the well--known Boltzmann distribution for the
level population densities
\begin{equation}
\frac{n_\mathrm{u}}{n_\mathrm{l}}=\frac{g_\mathrm{u}}{g_\mathrm{l}}\cdot
e^{-\frac{E_\mathrm{{u}}-E_\mathrm{{l}}}{kT_\mathrm{e}}}=\frac{g_\mathrm{u}}{g_\mathrm{l}}\cdot
e^{-\frac{h\nu}{kT_\mathrm{e}}} \label{Boltzmann}
\end{equation}

Local thermodynamic equilibrium represents the equilibrium between
particles. The velocities of ions and electrons are described by a
Maxwell distribution. Temperature $T_\mathrm{e}$ may vary from one
place to another, hence the name ``local''. The population density
is described by Boltzmann equation~\ref{Boltzmann} with a
temperature identical with that for the electron velocity
distribution. When we extend Boltzmann relation to continuum
states~\citep{Griem97} we can arrive the Saha equation
\begin{eqnarray}
\frac{n_\mathrm{e}n^{z+1}}{n^z}&=&2\frac{Q^{z+1}(T_\mathrm{e})}{Q^z(T_\mathrm{e})}
\left( \frac{2\pi
m_\mathrm{e}kT_\mathrm{e}}{h^{2}}\right)^{3/2} \mathrm{e}^{-\frac{E_{i}}{kT_\mathrm{e}}} \nonumber\\
\frac{n_\mathrm{e}n^{z+1}}{n^z}&=&6.10^{21}\frac{Q^{z+1}(T_\mathrm{e})}{Q^z(T_\mathrm{e})}T_\mathrm{e}^{3/2}\mathrm{e}^{-\frac{E_i}{T_\mathrm{e}}}\quad[\mathrm{eV;}\,\mathrm{cm}^{-3}]
\label{Saha}
\end{eqnarray}

that describes the total densities of adjacent ionization stages
$n^z$ and $n^{z+1}$. The term $+ze$ represents the ion charge.
$E_{i}$ stands for ionizing energy of an ion/atom with the density
$n^z$. $Q(T_e)$ is the partition function defined by
\begin{equation}
Q^z(T_\mathrm{e})=\sum_ig_i^z\cdot
\mathrm{e}^{-\frac{E_i-E_1}{kT_\mathrm{e}}}
\end{equation}

The sum goes over all bounded states $i$. The number of terms that
are included to evaluate the partition function depends not only
on the plasma temperature but also on the density.

The thermodynamic equilibrium is further described by the Planck
blackbody function for radiation energy with the same temperature
$T=T_\mathrm{e}$. This is no more valid in LTE where the radiation
density could be below the blackbody level.

\subsubsection{Validity conditions for local thermodynamic equilibrium}

The first necessary condition of LTE is a Maxwell distribution of
electron velocities.

Another condition is given by the validity of reducing
equation~\ref{quasiequilibrium} to equation~\ref{LTE1}. It means
that the unequality  $A_{u\rightarrow}\ll C_{u\rightarrow}$ has to
be satisfied. Usually a factor of ten is considered as
sufficiently high, i.e. $10\ A_{u\rightarrow}\leq
C_{u\rightarrow}$. Unfortunately it is impossible to derive any
easy criterion for \emph{complete} LTE (i.e. for the populations
of all levels). The review of C.~De~Michelis and M.~Mattioli
provides the necessary, but not sufficient,
criterion~\citep{deMichelis81}
\begin{equation}
n_\mathrm{e}\geq 1,8.10^{14}\sqrt{kT_\mathrm{e}}\Delta
E^3_\mathrm{ul} \quad [\mathrm{eV; cm}^{-3}]
\end{equation}

This criterion is difficult to satisfy especially for the largest
energy level difference $\Delta E_\mathrm{ul}$ in the level
scheme. Nevertheless, for any $n_\mathrm{e}$ the collisions still
dominate between high--lying levels. Level, above which excited
stated are in equilibrium with the ground state of the next
ionization stage, is called thermal limit. Then we said that
plasma is in \emph{partial} LTE. We use the following
criterion~\citep{Griem64}
\begin{equation}
n_\mathrm{e}\geq
7.10^{17}\frac{(z+1)^6}{n_{th}^{17/2}}\sqrt{\frac{kT_\mathrm{e}}{E_\mathrm{H}}}
\quad [\mathrm{eV; cm}^{-3}]
\end{equation}

that determines the minimal electron density $n_\mathrm{e}$ which
is needed for partial LTE of levels above the principal number
$n_\mathrm{TH}$. Here $z$~is the effective nuclear charge and
$E_\mathrm{H}\doteq13,6$ eV is the ionization energy of hydrogen.

Finally we can mention the importance of the relaxation time. It
is evident that the time necessary for making an equilibrium must
be substantially smaller than the characteristic time of processes
in plasma. More details about the conditions can be found
in~\citep{Griem64,Griem97,Thorne99}.


\subsection{Radiative transfer}

Until then we were interested in the influence of collisional and
radiative processes on the population of energy levels. It was
important since the population of energy level $n_\mathrm{u}$ and
the transition probability of spontaneous emission determines the
local emission in the plasma. The local emission is described by
the emissivity, the power emitted per unit solid angle per Hz by
unit volume
\begin{equation}
\epsilon_\nu=\frac{\diff^3 \Phi}{\diff V\diff \Omega\diff \nu}
\end{equation}

and
\begin{equation}
\epsilon_\nu(\mathrm{u}\rightarrow
\mathrm{l})=\frac{h\nu}{4\pi}A_{\mathrm{ul}}n_\mathrm{u}
\end{equation}

The importance of emissivity lies in the fact that it contains
information about local properties of the plasma. However, it is
impossible to directly determine the emissivity by passive
emission spectroscopy. We usually measured the spectral radiance
$L_\nu$ at the surface of plasma, the power emitted per unit solid
angle per Hz by unit projected area
\begin{equation}
L_\nu=\frac{\diff^3 \Phi}{\diff S \cos\theta \diff \Omega\diff
\nu}
\end{equation}

 The relation between these two quantities is trivial
only in the case of optically thin plasma where the absorption and
re-emission of photons are neglected. Otherwise we have to solve
the equation of radiative transport, which may be written for the
line of sight along the axis $x$
\begin{equation}
\label{radiativetransfer}
\diff L_{\nu}(\vec{r},\Omega)=\bigg[
\epsilon_{\nu}(\vec{r},\Omega)-\kappa(\nu,\vec{r})
L_{\nu}(\vec{r},\Omega)\bigg] \diff x
\end{equation}

Here $\kappa(\nu,\vec{r})$ represents the effective absorption
coefficient that could be negative if stimulated emission occurs.
We now define a quantity called the source function
$S_{\nu}(\vec{r})$ as the ratio of the emissivity to the
absorption coefficient
\begin{equation}
 S_{\nu}(\vec{r},\Omega)=\frac{\epsilon_{\nu}(\vec{r},\Omega)}{\kappa(\nu,\vec{r})}
\end{equation}

And by using the optical depth $\tau(\nu,\vec{r})$
\begin{equation}
\diff \tau(\nu,\vec{r})=\kappa(\nu,\vec{r})\diff x
\end{equation}

we can rewrite equation \ref{radiativetransfer} as follows
\begin{equation}
\frac{\diff L_{\nu}(\vec{r},\Omega)}{\diff
\tau(\nu,\vec{r})}=S_{\nu}(\vec{r},\Omega)-L_{\nu}(\vec{r},\Omega)
\end{equation}

Unfortunatelly this equation cannot be solved in general
(cf.~\citep{Aschke00, Kunze02}) because the emissivity and
absorption coefficient may have different spectral dependence.
Moreover, the absorption of photons influences the population of
energy levels and thus it is necessary to solve the equation
\ref{radiativetransfer} together with the system of
equations~\ref{rychlostnirovnice}.

The solution of equation~\ref{radiativetransfer} can be found only
in limiting cases. If we suppose the homogenous plasma with the
characteristic length along the line of sight $l_\Omega$ and the
spatially isotropic source function $S_{\nu}$ we can arrive at the
relation
\begin{equation}
L_{\nu}=S_{\nu}(1-\mathrm{e}^{-\tau(\nu)})
\end{equation}

where $\tau(\nu)=\int\diff \tau(\nu,\vec{r})=\kappa(\nu)
l_\Omega$.

Furthermore, if the plasma is optically thin \mbox{($\tau\ll 1$)},
i.e. without absorption,  we can use the Taylor series
$\mathrm{e}^{-\tau(\nu)}\approx 1-\tau(\nu)$. Then we obtain
\begin{equation}
L_{\nu}\approx\int\epsilon_{\nu}(\vec{r},\Omega)\diff
x=\epsilon_{\nu}l_\Omega
\end{equation}

In another limiting case $\tau\gg 1$, we can derive
\begin{equation}
L_{\nu}=S_{\nu}=\frac{\epsilon_{\nu}}{\kappa(\nu)}=\frac{2h\nu^3}{c^2}\cdot\frac{1}{e^{h\nu/kT}-1}
\end{equation}

The last equality is valid in the case of the plasma in
thermodynamic equilibrium. The limiting case $\tau\gg 1$ is not
reached in the entire spectral range. Since the absorption
increases with $\lambda^2$, the plasma becomes optically thick
towards long wavelength~\citep{Kunze89}. The emission lines become
optically thick more easily than continuum at short wavelengths.
From the experimental point of view it is necessary to know if the
spectral line is optically thick. For Doppler--broadened lines and
the plasma in LTE, the optical thickness at the line centre
$\nu_0=c/\lambda_0$ is given by
\begin{equation}
\tau(\nu_0)=r_\mathrm{B}\sqrt{\frac{\pi M_\mathrm{i}c^2}{2kT}
}\lambda_0f_{\mathrm{ul}}n_\mathrm{l} l_\Omega
\end{equation}

where $r_\mathrm{B}=e^2/4\pi\varepsilon_0m_\mathrm{e}c^2$ is the
classical (Bohr) electron radius. Substituting known constants in
the previous equation, we get the equation
\begin{equation}
\tau(\nu_0)\doteq1,08.10^{19}\sqrt{\frac{M_\mathrm{i}}{2kT}}
\lambda_0f_{ul}n_l l_\Omega
\end{equation}

Here the ion mass $M_\mathrm{i}$ is in atomic units
$m_\mathrm{u}$, temperature $kT$ in~eV, the population of lower
level $n_\mathrm{l}$ in~m$^{3}$, the wavelength $\lambda_0$ in~nm,
and the length of plasma $l_\Omega$ in~m.

Experimentally we can check if the emission lines are optically
thick or thin by comparing the relative intensities of close
multiplet lines. The radiance ratio of two optically thin
multiplet lines is determined by the statistical weights of lower
levels $g_\mathrm{l}$ and the oscillator strengths $f_\mathrm{lu}$
\begin{equation}
\frac{L_{\nu_1}}{L_{\nu_2}}=\frac{f_{\mathrm{l}_1\mathrm{u}_1}g_{\mathrm{l}_1}}{f_{\mathrm{l}_1\mathrm{u}_2}g_{\mathrm{l}_2}}
\end{equation}

If the measured ratio is higher in favor of the weaker line, the
spectral lines are not optically thin. As a result the temperature
cannot be easily determine by the intensity ratio of spectral
lines.

\subsubsection{Intensity of spectral lines}

The intensity of spectral line $I$ is often refereed in the
scientific literature. The fact of the matter is that the correct
term is the spectral radiance $L_\nu$, mostly spatially and/or
temporally integrated. As the intensity became common we will use
it in the following text in spite of that the spectral radiance is
more appropriate.

\subsection{Spectroscopic measurements of plasma parameters}

The emission spectroscopy of plasma belongs to one of the
fundamental passive diagnostic technique. The emissivity of plasma
contains a lot of information about plasma properties and
dynamics. The key issue is the choice of a suitable method which
enabled the estimation of plasma parameters, especially the
electron temperature and density. Our choice of a method was
predetermined by the properties of our grating spectrograph (see
subsection~\ref{spectrograph} on page~\pageref{spectrograph}). It
enables only the measurement of relative intensities of spectral
lines. The measurement of line profile was not possible due to
limited spectral resolution. That is why the manifold choice of
spectroscopic technique (cf. \citep{Griem64, Griem97,
deMichelis81}) reduces to several fundamental methods.

\subsubsection{Spectroscopic measurement of temperature and density}

First, it is important to remember that a spectroscopic
measurement of temperature is actually measurement of a parameter
determining some equilibrium distribution \citep{Thorne99}.
Therefore we can distinguish between the electron temperature
$T_\mathrm{e}$ and the ion temperature $T_\mathrm{i}$. Moreover we
can distinguish between the electron temperature occurring in the
Maxwell velocity distribution, in the Boltzmann
distribution~\ref{Boltzmann} (so-called population or excitation
temperature), in the Saha--Boltzmann equation~\ref{Saha}
(ionization temperature), and etc. Unless any equilibrium
distribution exists, the temperature is not defined and the plasma
have to be described by the distribution functions. Most of
spectroscopic temperature measurement primarily yield
$T_\mathrm{e}$. The same was in our case. The kind of the electron
temperature (excitation, ionization, etc.) follows from the method
used and will not be specified in our work.

\begin{itemize}
\item[--] Very easy and undemanding method of the rough
temperature measurement is the identification of ionic states in a
plasma. In order ro reach an ionic state with ionization potential
$E_\mathrm{i}$, the electron temperature must obey
\begin{equation}
\label{odhadteploty}
 T_\mathrm{e}>C_\mathrm{i} E_\mathrm{i}
\end{equation}

with $C_\mathrm{i}$ varying approximately between 0.1 and 0.3
\citep{Hauer91}.

More accurate value of temperature can be obtain from the
calculation of ionization equilibrium (the temperature dependence
of population of various ionic states). The free parameter in this
calculation is the electron or ion density. To calculate
ionization equilibrium we used atomic physics code FLY.

\item[--] Another common method is based on relative line
intensities of the same ion.

Provided the plasma is in LTE or at least in partial LTE, the
population of energy levels follows the Bolzmann
distribution~\ref{Boltzmann}. Then the ratio of two optically thin
spectral lines is given by
\begin{equation}
\label{ratio}
\frac{L_{\nu}}{L_{\nu'}}=\frac{A_\mathrm{ul}g_\mathrm{u}\lambda '}
{A_\mathrm{u'l'}g_\mathrm{u'}\lambda}\cdot
\mathrm{e}^{-(E_\mathrm{u}-E_\mathrm{u'})/kT_\mathrm{e}}
\end{equation}

It can be clearly seen from Eq.~\ref{ratio} that, besides several
constants, the ratio is dependent only the electron temperature.
The sufficient sensitivity is achieved for
$E_\mathrm{u}-E_\mathrm{u'}> kT_\mathrm{e}$. This method can be
extended to more spectral lines than two. We can make a graph with
$\ln (L_{\nu} \lambda/g_\mathrm{u} A_\mathrm{ul})$ on the
$x$--axis and with the energy of upper level $E_\mathrm{u}$ on the
$y$--axis. The slope of the line then equals $-T_\mathrm{e}$. This
method was used in cases when the code FLY cannot be applied, e.g.
for Be--like ions.

\item[--] In the regions where (partial) LTE approximation is no
more valid, the ratio of two spectral lines is not only
temperature-- but also density--dependent. In such circumstances a
detailed accounting must be made of the ionization, recombination,
excitation, deexcitation and radiative transfer. As far as this
work is concerned, we used the code FLY to calculate the
population of the states and the ratio of line intensities in
non--LTE approximation (usually in collisional--radiative
equilibrium). The suite FLY enables also the reconstruction of the
synthetic spectrum for a particular temperature and density. Since
the ratio of spectral lines is not only temperature dependent we
can estimate the density. It was very useful since the other
methods of density measurement (such as Stark broadening,
depression of ionization potential, Inglis--Teller limit, or the
ratio of resonance and intercombination lines of He--like ions)
cannot be applied.
\end{itemize}

